RMS-FlowNet: Efficient and Robust Multi-Scale Scene Flow Estimation for Large-Scale Point Clouds

The proposed RMS-FlowNet is a novel end-to-end learning-based architecture for accurate and efficient scene flow estimation which can operate on point clouds of high density. For hierarchical scene flow estimation, the existing methods depend on either expensive Farthest-Point-Sampling (FPS) or structure-based scaling which decrease their ability to handle a large number of points. Unlike these methods, we base our fully supervised architecture on Random-Sampling (RS) for multiscale scene flow prediction. To this end, we propose a novel flow embedding design which can predict more robust scene flow in conjunction with RS. Exhibiting high accuracy, our RMS-FlowNet provides a faster prediction than state-of-the-art methods and works efficiently on consecutive dense point clouds of more than 250K points at once. Our comprehensive experiments verify the accuracy of RMS-FlowNet on the established FlyingThings3D data set with different point cloud densities and validate our design choices. Additionally, we show that our model presents a competitive ability to generalize towards the real-world scenes of KITTI data set without fine-tuning.

==> tables/Table3.tex <==
\begin{table}[b]
	\caption{Comparing \gls{fps} and \gls{rs} with our architecture. Both variants are tested on 8192 points. \Gls{fps} performs slightly better accuracy on \gls{ft3d} and stronger generalization on KITTI at the cost of efficiency (memory and run-time). This proofs the universal capability of our Flow-Embedding.}
	\label{Table3_Sampling}
	\begin{center}
		\resizebox{1.0\linewidth}{!}
		{
			\begin{tabular}{c|cccc|cc}
				\multirow{3}{*}{\textbf{Sampling}}  
				& \multicolumn{2}{c}{\multirow{1}{*}{\textbf{\acrshort{ft3d_bold} \cite{mayer2016large}}}} 
				& \multicolumn{2}{c|}{\multirow{1}{*}{\textbf{KITTI \cite{menze2015object}}}} &  & \\ 
				
				& \textbf{EPE3D} & \textbf{Acc3DR} & \textbf{EPE3D} & \textbf{Acc3DR} & \textbf{GPU} & \textbf{Time} \Tstrut\Bstrut\\
				
				& [m] & [\%] & [m]  & [\%] & [GB] & [ms] \Tstrut\Bstrut\\
				\hline		
				FPS & \textbf{0.052} & \textbf{0.951} & \textbf{0.051} & \textbf{0.951} & 10.6 & 123 \Tstrut\Bstrut\\
				\textbf{RS} & 0.055 & 0.942 & 0.067 & 0.894 & \textbf{4.76} & \textbf{62} \Tstrut\Bstrut\\						
			\end{tabular}
		}
	\end{center}
\end{table}

